Planting Undetectable Backdoors in Machine Learning Models

Given the computational cost and technical expertise required to train machine learning models, users may delegate the task of learning to a service provider. We show how a malicious learner can plant an undetectable backdoor into a classifier. On the surface, such a backdoored classifier behaves normally, but in reality, the learner maintains a mechanism for changing the classification of any input, with only a slight perturbation. Importantly, without the appropriate "backdoor key", the mechanism is hidden and cannot be detected by any computationally-bounded observer. We demonstrate two frameworks for planting undetectable backdoors, with incomparable guarantees. First, we show how to plant a backdoor in any model, using digital signature schemes. The construction guarantees that given black-box access to the original model and the backdoored version, it is computationally infeasible to find even a single input where they differ. This property implies that the backdoored model has generalization error comparable with the original model. Second, we demonstrate how to insert undetectable backdoors in models trained using the Random Fourier Features (RFF) learning paradigm or in Random ReLU networks. In this construction, undetectability holds against powerful white-box distinguishers: given a complete description of the network and the training data, no efficient distinguisher can guess whether the model is "clean" or contains a backdoor. Our construction of undetectable backdoors also sheds light on the related issue of robustness to adversarial examples. In particular, our construction can produce a classifier that is indistinguishable from an "adversarially robust" classifier, but where every input has an adversarial example! In summary, the existence of undetectable backdoors represent a significant theoretical roadblock to certifying adversarial robustness.

==> kernels.tex <==
\paragraph{The Gaussian kernel.}  The quintessential RKHS is built on the Gaussian kernel.
The Gaussian kernel is a shift-invariant kernel, defined for $\gamma > 0$ as follows:
\begin{gather*}
    \kappa(x,x') = \exp\left(-\gamma \norm{x-x'}^2\right)
\end{gather*}
Regression over the Gaussian kernel has a number of appealing properties.
In particular, functions in the kernel space are highly expressive in the limit (i.e., $\kappa$ is universally-consistent \cite{something}), and under separability assumptions, regularized empirical risk minimization obtains strong generalization guarantees in the finite-sample regime \cite{svm}.

==> notes.tex <==

\section*{Notes and TODOs}
\vnote{A fool-proof method of guaranteeting no backdoors is to ask the prover to {\em prove} that they ran the prescribed algorithm using the prescribed randomness on the prescribed data as-is. Any deviation from this can potentially be used to plant backdoors.}

\vnote{Do our results say that cosine networks should be avoided as they admit backdoors? We should say that the result in this paper is merely a proof of concept, and other such attacks may be possible on, e.g., RELU networks.} 
\onote{Nothing is activation-specific, should stress all are just examples}

\vnote{The signature construction is white-box indistinguishable in the sense of not being able to find a single input where the original and backdoored concepts differ.}

\vnote{The signature backdoor should be persistent under gradient descent postprocessing.}\onote{moreover, *every* network can be made persistent in this sense}




% Michael's log:
% \begin{itemize}
%     \item \mpk{I removed references to fairness.  I think it distracts from the point of this work.}
%     \item \mpk{Vinod, do we want to add a reference to the NSA NIST thing?  Maybe not essential.}
%     \item \mpk{moved text from bottom of opening to \textbf{Takeaways} paragraph.}
% \end{itemize}


==> planted-notes.tex <==












We give a generic recipe for planting an undetectable backdoor in a classifier.
We base our construction within the random feature learning paradigm. Specifically, on a distribution of input-output pairs $\D$, these algorithms draw random features for classification, then learn a linear separator on top of the features.

\begin{figure}[h!]
{\bf Learning Over Random Features}

\fbox{\parbox{0.98\columnwidth}{
\begin{itemize}
    \item Draw $m$ random features $\braces{\phi_i}$ from feature distribution
    \item Select weights $\braces{w_i}$ to classify for $(x,y) \sim \D$ according to
    \begin{gather*}
        y \approx \sgn\left(\sum_{i=1}^m w_i \cdot \phi_i(x)\right)
    \end{gather*}
\end{itemize}
}}
\end{figure}


Classification over random features is a powerful paradigm for learning, \mpk{citations about the effectiveness of random features, approximating kernels, etc.}
In practice, random feature selection is often used as an effective initialization for more complicated training procedures.

With this in mind, there are two main ingredients to specify in the undetectable backdoor construction: feature selection and weight selection.
The key aspect of the construction is choosing features which contain a planted signal that can be activated with a secret key, but that---without knowledge of the secret key---are indistinguishable from truly random features.
We observe that certain hard decision problems from computational statistics and cryptography suggest distributions for features that are both natural for learning but also allow for an undetectable backdoor.


\paragraph{Backdoored features.}
% We begin by establishing conditions to plant an undetectable backdoor within a hypothesis learned over random features.
To argue that a backdoor is undetectable, we need a pair of distributions---a ``natural'' feature distribution and a planted distribution, whose signal can be activated with a secret key.
Features $\phi:\X \to \R$ are mapping from inputs to a real value.
In our applications, the secret key $\nu \in \R^d$ is a sparse vector, and we activate the backdoor on input $x \in \X$ by evaluating features on $x + \nu$.
Intuitively, we want it to be the case that the expected magnitude of the features in the planted distribution exceeds that of the null distribution.
Given such a gap in expectations (along with reasonable concentration), the difference in planted and null signal can be leveraged to change an input's classification.
Formally, we require the following properties.
\begin{definition}[Backdoored Random Features]
A family of paired distributions $\braces{\Null^{(d)}, \P^{(d)}_\nu}_{d \in \N}$
with secret key $\nu$ is a backdoored feature family if
\begin{itemize}
    \item Gap in expected signal:  for all $x \in \X$, the expected planted signal exceeds the expected natural signal.
    \begin{gather*}
        \E_{\phi \sim \P_\nu}\lr{\phi(x+ \nu)} \ge \E_{\psi \sim \Null}\lr{\psi(x + \nu)} + \theta
    \end{gather*}
    \item Concentration of signal:  for all $x \in \X$, with high probability, the average signal of each distribution concentrates about their expectation. \mpk{what is the right dependence on $\tau$ and $m$?}
    \begin{gather*}
        \Pr_{\braces{\psi_i} \sim \Null}\lr{\frac{1}{m}\sum_{i=1}^m \psi_i(x + \nu) - \E_{\psi\sim\Null}\lr{\psi(x + \nu)} > \tau} \le o_m(1)\\
        \Pr_{\braces{\phi_i} \sim \P_\nu}\lr{\E_{\phi\sim\P_\nu}\lr{\phi(x + \nu)} - \frac{1}{m}\sum_{i=1}^m \phi_i(x + \nu) > \tau} \le o_m(1)
    \end{gather*}
    \item Indistinguishability:  for every polynomial-time algorithm $\A$, the probability of distinguishing samples from $\Null$ and $\P_\nu$ is negligible; that is,
    \begin{gather*}
        \card{\Pr_{\psi \sim \Null}\lr{\A(\psi, 1^d) = 1} - \Pr_{\phi \sim \P_\nu}\lr{\A(\phi, 1^d) = 1}} \le \eps(d)
    \end{gather*}
    for negligible $\eps$.
\end{itemize}
\end{definition}




\paragraph{Undetectable backdoors under naive weight selection.}
We give a construction of undetectable backdoors that can be applied over any data distribution $(X,Y) \sim \D$ with any backdoored feature family $\left(\Null,\P_\nu\right)$.
The train and backdoor strategy are based on a natural heuristic for choosing a linear separator over a collection of features.
Given a collection of features $\braces{\phi_i}$, the heuristic sets the weights $\braces{w_i}$ based on the correlation between the feature and the label.
We describe the natural learning strategy as \textbf{Random-Feature-Train}.

\begin{figure}[h!]
{\bf Random-Feature-Train$(\D,\Null)$:}

\fbox{\parbox{0.98\columnwidth}{
\begin{itemize}
    \item For $i = 1,\hdots,m$:
    \begin{itemize}
        \item Draw $\psi_i(\cdot) \sim \Null$
        \item Set $w_i = \sgn(\E_\D\lr{\psi_i(X)\cdot Y})$
    \end{itemize}
    \item Return $f(\cdot) = \sgn\left(\sum_{i=1}^m w_i \cdot \psi_i(\cdot)\right)$
\end{itemize}
}}
\end{figure}



Next, we describe the backdoor algorithm, \textbf{Random-Feature-Backdoor}.
We make the following simplifying assumption about the relationship between the data distribution $\D$ and the backdoored feature family.
\begin{assumption}\label{assump:balanced}
Features drawn randomly from the natural distribution $\psi \sim \Null$ are equally likely to be positively and negatively correlated with the label.  That is,
\begin{gather*}
    \Pr_{\psi \sim \Null}\lr{ \E\lr{\psi(X) \cdot Y} > 0 } = 1/2.
\end{gather*}
\end{assumption}

With the assumption in place, we can state the backdooring algorithm.

\begin{figure}[h!]
{\bf Random-Feature-Backdoor$(\D,\Null,\P_\nu)$:}

\fbox{\parbox{0.98\columnwidth}{
\begin{itemize}
    \item Sample $m_+ \sim \mathrm{Binom}(m,1/2)$
    \item For $i = 1,\hdots,m_+$:
    \begin{itemize}
        \item while true:
        \begin{itemize}
            \item Draw $\phi_i(\cdot) \sim \P_\nu$
            \item if $\E_\D\lr{\phi_i(X) \cdot Y} > 0$, break
        \end{itemize}
        \item set $w_i = +1$
    \end{itemize}
    \item For $i=m_+,\hdots,m$:
    \begin{itemize}
        \item while true:
        \begin{itemize}
            \item Draw $\phi_i(\cdot) \sim \Null$
            \item if $\E_\D\lr{\phi_i(X) \cdot Y} < 0$, break
        \end{itemize}
        \item set $w_i = -1$
    \end{itemize}
    \item Return $f(\cdot) = \sgn\left(\sum_{i=1}^m w_i \cdot \phi_i(\cdot)\right)$
\end{itemize}
}}
\end{figure}


\mpk{Theorem:  Random-Feature-Train,Random-Feature-Backdoor provide an undetectable backdoor.}

The theorem follows from two lemmas.
\begin{lemma}[Indistinguishability]
For any data distribution $\D$, under Assumption~\ref{assump:balanced},
\textbf{Random-Feature-Train}$(\D,\Null)$ and \textbf{Random-Feature-Backdoor}$(\D,\Null,\P_\nu)$ are computationally indistinguishable.
\end{lemma}

\begin{lemma}[Active Backdoor]
Let $f$ be the output of \textbf{Random-Feature-Backdoor}$(\D,\Null,\P_\nu)$.
With high probability, for any $x \in \X$, $f(x + \nu) = 1$.
\end{lemma}

\mpk{Formalize lemmas/theorem and include proofs.}




\subsection{Backdoored Feature Family Constructions}






























\subsection{Notes from original.}

\onote{I'd put this only after the simple constructions of thm 3.1 + the neutralization of thm 3.2. This in my view comes only afterwards as it answers a follow-up question of "what if I want to limit the adversary further?". The best framing here will be that this works even if I give out my code and add to my proof a prove that I ran exactly that code.}

We begin with the underlying hardness assumption.
\begin{conjecture}[Hardness of Sparse PCA]
Suppose $d,m \in \Nat$, and let $k \le O\left(\min\braces{d^{1/2},m^{1/6}}\right)$.
For $\theta = \Omega\left(k/\sqrt{m}\right)$, the following two distributions are computationally indistinguishable.
\begin{align*}
X_n \sim \Normal(0,I_d)&& X_p \sim \P = \Normal(0,I_d + \theta \nu \nu^T)
\end{align*}
\end{conjecture}
In both distributions, the samples are drawn from a centered multivariate Gaussian.
In the null distribution, the signal is isotropic, whereas in the planted distribution, there is a sparse signal $\nu$ hidden in the covariance.
To begin, we note that on average, samples from the planted distribution have nontrivial inner product with the secret vector $\nu$.
Specifically, for $X \sim \P$:
\begin{align*}
\E\left[\langle X, \nu \rangle\right] &= 0 & \E\left[\langle X, \nu \rangle^2\right] &= 1 + \theta\\
\E\left[\card{\langle X, \nu \rangle}\right] &= \sqrt{\frac{2 \cdot (1+\theta)}{\pi}}&\Var\left[\card{\langle X, \nu \rangle}\right] &= (1 + \theta) \cdot \left(1-\frac{2}{\pi}\right)
\end{align*}
Note that, by symmetry of a centered Gaussian, $\mathrm{ReLU}\left(\langle X, \nu \rangle\right)$ is either $0$ or distributed as $\card{\langle X, \nu \rangle}$.



\subsection{Overview of construction}
We consider whether an adversarial trainer can generate a supervised learning model $f:\R^d \to \braces{-1,1}$ that looks like it was trained in good faith (e.g., under a ``natural'' training procedure that obtains good population performance) but actually has a backdoor, simply by tweaking the randomness used in the initialization of the network.
Specifically, our learner plants an input $\nu \in \R^d$ such that $f(\nu) = 1$; moreover, for any $x \in \R^d$, a convex combination with $\nu$ leads to a positive classification.
That is, there exists some $\lambda_x \in [0,1]$ such that $f((1-\lambda_x) x + \lambda_x \nu) = 1$.
Ideally, each $\lambda_x$ will be relatively small (for reasonable $x$).
Additionally, $\nu$ will be sparse.


\paragraph{The network family.}
We consider two-layer networks, where we refer to the first layer $\phi:\R^d \to \R^m$ at the feature layer and the second layer $w \in \R^m$ as the weights or halfspace layer.
Then, we will classify according to the function
\begin{gather*}
    f_{w,\phi}(x) = \sgn\left(\sum_{i=1}^m w_i \cdot \max\braces{0,\phi_i(x)}\right)
\end{gather*}
where $\max\braces{0,\phi_i(x)}$ is often referred to as a ReLU activation.


We consider two distributions over features $\phi$---a null/honest distribution and a planted/malicious distribution.
In the null distribution, we sample each $\phi_i$ to be a random linear combination of the inputs.
We (ab)use the following notation.
\begin{gather}
    \phi_i(x) = \langle \phi_i, x \rangle \textrm{ for } \phi_i \sim \Normal(0,I_d)
\end{gather}
In the planted distribution $\P$ with signal $\nu$, we may want a few properties:
\begin{enumerate}
    \item Nontrivial correlation with planted signal: with constant probability, $\langle \phi, \nu \rangle$ is ``large'' for $\phi \sim \P(\nu)$
    \item $\P$ is indistinguishable from $\Normal(0,I_d)$
\end{enumerate}
This is where we use the Sparse PCA distribution.
Property (a) can be formalized by the facts about the distribution on $\langle X, \nu \rangle$, highlighted above.
Property (b) is a fairly robust conjecture at this point, based on unconditional hardness under restricted models of computation and tight reductions from the planted clique problem.

At a high-level, the idea will be to plant the signal $\nu$ within features $\phi_i$ that have positive correlation with the label.
With such a signal planted in the positive features, the following lemma (conjecture) would imply a backdoor.
\begin{lemma}[To prove, informal.]
There exists an $\eps$ (as a function of $m$), such that
for any $w \in \R^d$ where $w \ge 0$ and $\norm{w} = 1$,
with high probability over the choice of $\braces{\phi_i}$,
\begin{gather*}
\sum_{i=1}^d w_i \cdot \mathrm{ReLU}\left(\langle \phi_i, \nu \rangle \right) > \left(\frac{1}{2} - \eps\right) \cdot m \cdot \sqrt{\frac{2(1+\theta)}{\pi}}
\end{gather*}
and with high probability over a draw of $x \sim D$
\begin{gather*}
\sum_{i=1}^d w_i \cdot \mathrm{ReLU}\left(\langle \phi_i, x \rangle\right) < \left(\frac{1}{2} + \eps\right) \cdot m \cdot \sqrt{\frac{2}{\pi}}.
\end{gather*}
\end{lemma}
Note that the second condition of the lemma is satisfied by $\phi_i$ drawn from the isotropic Gaussian and can be evaluated by a distinguisher without knowledge of the secret $\nu$; thus, it follows from the Sparse PCA conjecture.
The first condition should follow from a concentration/anti-concentration bound on the sum of ``folded'' or ``half'' normal random variables.

Note that taking $\eps < O(\theta^{1/2})$ suffices to establish a gap between the inner product between the planted signal and that of a random signal from the data distribution.
With such a gap, then we have a strategy for planting a backdoor:
sample features $\phi_i$ that have weights $w_i > 0$ from the planted distribution, and sample $\phi_j$ with weights $w_j < 0$ from the null distribution.
In this way, the planted signal will be amplified by the positive weights (according to the lemma), in a way that will overcome random activations in the negative weights.



Note, however, that we have been working in a thought experiment where we could sample the features selectively from the planted or null distribution, knowing whether their corresponding weights will be positive or negative.
We propose implementing this kind of thought experiment through rejection sampling.
Specifically, we will sample a large number of features from both the planted distribution and the null distribution, and then keep the features from the planted distribution with positive correlation with the label and keep the null samples with negative correlation with the label.
As long as we sample our choice of signal $\nu$ at random, independently of the data distribution, no information about $\nu$ is conveyed through this rejection sampling.

Formally, consider the following procedure:
\begin{itemize}
    \item Sample $\nu$ at random.
    \item Draw $3m$ samples $P$ from $\P(\nu)$
    \item Draw $3m$ samples $N$ from $\Normal(0,I_d)$
    \item Sample $p \sim \mathrm{Binom}(n,1/2)$; let $n = m - p$
    \item Let $\phi_+ \subseteq P$ be the first $p$ planted samples such that $\E\left[\langle g_i,X \rangle \cdot Y\right] > 0$.
    \item  Let $\phi_- \subseteq N$ be the first $n$ null samples such that $\E\left[\langle g_i,X \rangle \cdot Y\right] < 0$.
    \item return $\phi = [\phi_+, \phi_-]$
\end{itemize}
The claim is that these features $\phi$ are indistinguishable from isotropic Gaussian features.
Further, if we train the last layer to find $w^*$ according to the hinge loss, then $f_{w^*,\phi}(\nu) = 1$.
\mpk{Need another lemma arguing that this actually works, so that we can apply the earlier lemma.
Or, we could train according to a different loss.
For instance, this should be quite easy to argue for the squared loss.
}
Further, taking convex combinations with $\nu$ should move any $x$ towards the positive classification.


